A Skeleton-Driven Neural Occupancy Representation for Articulated Hands

We present Hand ArticuLated Occupancy (HALO), a novel representation of articulated hands that bridges the advantages of 3D keypoints and neural implicit surfaces and can be used in end-to-end trainable architectures. Unlike existing statistical parametric hand models (e.g.~MANO), HALO directly leverages 3D joint skeleton as input and produces a neural occupancy volume representing the posed hand surface. The key benefits of HALO are (1) it is driven by 3D key points, which have benefits in terms of accuracy and are easier to learn for neural networks than the latent hand-model parameters; (2) it provides a differentiable volumetric occupancy representation of the posed hand; (3) it can be trained end-to-end, allowing the formulation of losses on the hand surface that benefit the learning of 3D keypoints. We demonstrate the applicability of HALO to the task of conditional generation of hands that grasp 3D objects. The differentiable nature of HALO is shown to improve the quality of the synthesized hands both in terms of physical plausibility and user preference.

==> old-Sec1-intro.tex <==
\section{intro}
\KK{OLD TEXT}

Capturing the dense surface of hands is crucial for many applications that need to reason about contact in detail. For example, to accurately model grabbing a virtual object in VR or AR the precise surface of the user's hand needs to be represented. 
\KK{need more overview about contact and grasp here}
... Maybe put the work about capturing data with contact here (like ContactPose) ...



\KK{Explicit Model}
In order to generate grasp conditioned on a given object, prior works often rely on predicting parameters of an explicit hand model \cite{corona2020ganhand,GRAB2020}.
Such prediction leverages the underlining pose and shape prior of the hand model to guide the model to generate valid hand poses.
While yielding encouraging initial results, mesh-based approaches are not without limitations. Parametric representations tend to be less accurate than keypoint-based approaches and have reduced representation power since they typically require strong regularization of their parameters when fit to data. 
As such, a pose-processing step such as optimization \cite{corona2020ganhand} or refinement \cite{GRAB2020} is employed to improve the contact prediction between hand and object.
Furthermore, explicit representations themselves still have pitfalls. For instance, the amount of detail that can be represented is inherently limited by the mesh resolution, and mesh deformation need to be pre-defined. In addition, performing intersection tests, which is crucial for modeling hand interactions with objects \cite{hasson2019obman} or other hands \cite{Moon_2020_ECCV_InterHand2.6M}, can be cumbersome with explicit surface representations.







\KK{Implicit Function}
We observe that in other areas of computer vision, neural implicit representations for rigid 3D objects have gained traction \cite{mescheder2019occupancy, park2019deepsdf}.
Such representations have several advantages.
For example, they are continuous and therefore very flexible in modeling 
different shapes and topologies.
Moreover, neural representations can be learned without explicit 3D groundtruth via differentiable rendering~\cite{niemeyer2020differentiable}. 
In addition, they allow for efficient intersection tests, which is crucial for modeling interaction and contact between hands and objects. 
However, most of the existing neural implicit models have been designed with rigid objects in mind and tend to not generalize to deformable objects which makes them unsuitable for the case of 3D articulated objects such as human bodies and hands. 
A notable exception is NASA \cite{deng2020neural}, which represents human bodies with neural occupancy networks. While demonstrating initial feasibility, their model can only represent a single human subject and does not generalize well across different subjects, significantly limiting the applicability of the representation.
In the context of grasp generation, \cite{karunratanakul2020grasping} produce a label for each surface point to indicate the hand part. The part labels are then used for fitting the hand model to the predicted surface to obtain a valid hand mesh.


\KK{What we do. Too long - summarize}
In this work, we take inspiration from NASA \cite{deng2020neural} and propose {\methodnamefull}, a fully differentiable and  articulated  occupancy  representation for hands that generalizes well to a large variety of hand poses and shapes .
Making implicit representations applicable to the case of articulated hands is non-trivial and several challenges have to be overcome. First, the 3D shape of the hand is very sensitive to the kinematic structure and varies significantly across subjects. 
To address this issue we explicitly model the kinematic bone structure and propose constraints to encode bone lengths. We show that this helps in capturing the shape-dependent geometric deformations.
Second, most hand pose datasets use 3D Keypoints to represent the human hand. To make {\methodname} compatible with such 3D keypoint representations, we propose a novel differentiable layer that converts 3D hand poses to transformation matrices in a single forward pass. Importantly, this layer does not rely on iterative fitting such as inverse kinematics and can therefore be used without issue in back-propagation-based learning.
Since the transformation matrices define the mapping of the location and the orientation of each bone between articulated pose and the canonical pose space, this layer enables learning of an implicit template hand shape in the canonical space, and poses the template using the inverse of the transformation matrices to attain the final occupancy representation.


\KK{What we do. Details}
Using the propose implicit hand model, we generate grasp by using keypoints as a proxy for the full hand surface.
This formulation reduces the complexity of predicting the dense surface to just predicting the key points and allow more control over the pose and shape space. \KK{how to show?}.
Our generative model consists of two parts that can be trained both separately or jointly: the key point generator and the implicit hand model from key points.
To produce the rough pose and shape estimation, we first train the key point generation VAE conditioned on an object point cloud.
Then, to incorporate surface information, we attach the HALO model to the VAE to compute the surface contact loss. Because the HALO model is differentiable, the loss from the dense surface can propagate back to improve the keypoint model
As a result, our model can produce hand pose and surface in a unified manner without refinement or post-processing step to ensure contact.
\KK{optional} With our formulation, after the model is learned, we can also swap the implicit hand model with the explicit one to improve the prediction speed. We show that this method produce better result than learning to predict the parameter of such explicit model directly (without post-processing, of course).


\KK{Intro Summary}
In summary, we contribute:
\begin{enumerate}
  \item An articulated hand implicit surface representation that can generalized to different shapes;
  \item A differentiable layer that converts 3D skeleton to any canonical pose and produces bone transformation matrices based on a bio-mechanical assumption;
  \item A neural hand model that bridges the skeleton to the hand surface by taking in the commonly used 3D joints input and outputting an implicit surface
  \item We show the value of our keypoints-to-surface model in the grasp generation task where we decouple the pose generator from the complex hand model parameter space.
\end{enumerate}


==> old-Sec2-relatedWork.tex <==
The surface of the 3D hand can be represented both via explicit representations such as meshes or via implicit surfaces, parameterized by neural networks.
We defer the discussion on the implicit surface representation and discuss the more wildly used mesh-based representation here.
The use of explicit representation can be categorized into two approaches, MANO-based regression or dense surface regression, both of which transform a template mesh to the target pose but differ on how the poses are represented.
For parametric approaches, the hand pose and shape are represented via learned parameters, for example in PCA space. 
MANO \cite{MANO2017} and DeepHandMesh \cite{moon2020deephandmesh} both fall into this category.
Using the learned parameters implicitly induces a prior over poses upon the predictive model, however, it also increases the learning complexity as these features do not correspond directly to features in the inputs.
In addition, its representation space is also limited due to the regularization imposed on the parameter space.
Examples of works that utilize this approach include \cite{baek2019pushing,boukhayma20193d,hasson2020leveraging,hasson2019learning,zhang2019end}, where the MANO parameters are predicted directly using additional weak supervision such as hand masks \cite{baek2019pushing,zhang2019end} or 2D annotations \cite{boukhayma20193d,zhang2019end}.

Another way of utilizing explicit 3D hand models is to directly regress the dense vertices of a surface that represents the 3D hand \cite{ge20193d,Kulon_2020_CVPR,Moon_2020_ECCV_I2L-MeshNet}.
While more generalizable by avoiding constraints on the parameter space, this requires the corresponding dense 3D annotations which might be difficult, cumbersome, and costly to acquire. 
Ge et al.~\cite{ge20193d} leverage a synthetic dataset to acquire mesh annotations, Kulon et al.~\cite{Kulon_2020_CVPR} also predict the vertex locations directly via spiral-convolution but revert to supervision via MANO which may limit the expressivity of the approach.  
Our work differs in that we allow hand reconstruction from 3D keypoints as input and thus allow estimators to leverage direct image evidence. We eliminate the need for learning custom parameter spaces or predicting of dense surface points.




==> old-Sec3-method.tex <==
\subsubsection{Converting 3D Keypoints to bone transformations} \label{sec:bio_mech}


For {\methodname} to be useful for the task of 3D hand pose estimation, it is necessary to interface the underlying transformation matrices $\boldsymbol{B}_b$ with the 3D keypoint representation that is commonly used in the hand pose estimation literature. To learn a meaningful surface representation under articulation, it is necessary to convert between the articulated pose and the canonical pose in a \emph{consistent} manner. To this end, we note that simply converting 3D keypoints to a joint-angle representation is insufficient since the bones are not constraint with respect to rotation about themselves. Furthermore, to be able to leverage the resulting representation in end-to-end frameworks this conversion mechanism must be differentiable, ruling out iterative techniques such as inverse kinematics.  

Furthermore, to be able to leverage the resulting representation in end-to-end frameworks this conversion mechanism must be differentiable, ruling out iterative techniques such as inverse kinematics.   




\textbf{Notations.}
Given a hand skeleton represented by 3D key points $\boldsymbol{J}: \mathbb{R}^{21 \times 3}$, we denote
$\theta^f_{i}$ and $\theta^a_{i}$ to be the flexion and abduction angle of bone $i$ relative to its parent $p(i)$; 
$\theta^p_{i}$ to be the angle between a palmar bone $i$ and its adjacent palmar bone $i+1$; $\theta^n_{i}$ to be the plane angle between plane $n_i$ and $n_{i+1}$ spanned by the palmar bone $i-1$, $i$, $i+1$. We denote the properties of the reference canonical hand with $\prescript{c}{}{(.)}$


\subsubsection{bmc}

\noindent\textbf{Rotations to the Canonical Pose ($\boldsymbol{R^c}$)}
Given a local coordinate system $\boldsymbol{F}_i = (x_i, y_i, z_i)$ where $(x_i, y_i, z_i)$ are the axis of the coordinate system, for a bone $b_i$, we can measure the flexion angle $\theta^f_i$ and the abduction angle $\theta^a_i$ that characterize bone $i$ with respect to $\boldsymbol{F}_i$. Fig. \ref{fig: angles_coords} visualizes the local coordinate system $\boldsymbol{F}_i$ and how rotation angles are measured.
Then, given a canonical pose bone $b_i^c$, we compute the rotation matrix $\boldsymbol{R}^c_i$ to transform $b_i$ to its canonical pose $b_i^c$ based on the angles relative to the canonical pose $(\bar{\theta}^f_{i}$, $\bar{\theta}^a_{i})$ in $\boldsymbol{F}_i$.


\noindent\textbf{Angles to the Canonical Pose ($\bar{\theta}^f_{i}$, $\bar{\theta}^a_{i}$).}
Since the angles are measured in a consistent coordinate frame, to obtain the angle needed to rotate to the canonical pose,
we simply offset the angles of $b_i$ by the angle of $b_i^c$ in the canonical pose:
\begin{equation}
    \begin{aligned}
        \bar{\theta}^f_{i} &:= -\theta^f_{i} + \theta^f_{i_c} \\
        \bar{\theta}^a_{i} &:= -\theta^a_{i} + \theta^a_{i_c}  
    \end{aligned} \label{eq:angle2}
\end{equation}
where $\theta^f_{i_c}$ and $\theta^a_{i_c}$ are the flexion and abduction angle of the canonical pose with respect to $\boldsymbol{F}_i$. In our experiments, we use the canonical pose identical to that of MANO \cite{MANO2017}.

\noindent\textbf{Local Coordinate Frame to Global ($\boldsymbol{F'}$).}
Each rotation matrix $\boldsymbol{R}^c_i$ is defined locally with respect to a coordinate frame $\boldsymbol{F}_i$. The accumulated rotations $\boldsymbol{G}_i$ with respect to the root of the hand for a bone $b_i$ is then the product of the rotation matrices along the kinematic chain:
\begin{equation}
\boldsymbol{\boldsymbol{G}_{i}} =
    \begin{cases}
         \boldsymbol{G}_{p(i)} \boldsymbol{R}^c_{i} &\text{if } b_i \text{ is not a root bone}\\ %
         \boldsymbol{I}(4) &\text{otherwise.}
    \end{cases}
\end{equation}
Where $\boldsymbol{G}_{p(i)}$ are the rotations up to the parent of $b_i$. 
With the accumulated rotation matrices encoding the joint-angles relative to the palm of the hand, we need to map all matrices to global coordinates by multiplying with $\boldsymbol{F}_i^{-1}$. Recall that $\boldsymbol{F}_i$ encodes the mapping from the global coordinate system to the local frame. Thus, its inverse brings the angles back to the global coordinate frame. We summarize the accumulation of angles and the mapping to the global coordinate with the matrix $\boldsymbol{F}_i'$:

\begin{equation}
    \begin{aligned}
\boldsymbol{F}_i'      &=   \boldsymbol{F}_i^{-1} \boldsymbol{G}_{p(i)}.
    \end{aligned}
\end{equation}

With all the necessary components in place, we can compute the transformation matrices $\boldsymbol{B}^{-1}$ for all bones using only the 3D keypoints $\boldsymbol{J}$ in a differentiable manner. In Sec. \ref{sec:exp_3dkps} we show that the matrices derived using this formulation can be uses to recover hand surfaces that are very close to those attained by the ground truth transformation matrices from MANO.





\subsection{OLD TEXT}
\KK{OLD TEXT} \\
\KK{write down the math - let me and your coauthors check them. You should also have a draft experiments where you explain the data, metrics, baselines and your initial result (which doesn’t need to be better than baseline)}


\KK{Start methods - HALO method copied from CVPR submission}
In this section, we detail all the components necessary to attain a learnable implicit surface representation that applies to articulated hands under a wide variety of pose and shape induced deformation. We also derive a method to interface {\methodname} with the 3D keypoint representation that is commonly used in the hand pose estimation literature. Crucially our method is fully differentiable, opening the possibility of end-to-end trainable methods.  

HALO encompasses several aspects, schematically illustrated in Fig. \ref{fig: pipeline}. At inference time our model takes a hand pose encoded by 3D keypoints as input and converts these to a set of valid bone transformation matrices $\boldsymbol{B}$. These matrices are necessary to transform the bones of the hand back and forth between the canonical and the articulated pose. 3D query points $x$ from a volume surrounding the hand are mapped to the canonical space $\boldsymbol{B}^{-1}x$ in which the template shape of the hand is learned and stored in a neural implicit representation. 
Since each part of the hand induces deformation dependent displacements, following \cite{deng2020neural}, we use a separate implicit function to learn the local shape of each part of the hand (shown in different colors) in the output. The final output (here a mesh used for rendering only) is obtained via the marching cube algorithm.




\subsection{Preliminaries}
\KK{MANO to supp mat. HALO to merge with 3.2}
We first discuss two important building blocks for our method: MANO and Neural Articulated Shape Approximation (NASA).
From MANO we leverage the use of piece-wise rigid bone transformations and how to use these to transform a template mesh to a target configuration. From NASA we leverage the approach to learn an implicit surface representation via an array of per-bone neural networks to model pose and shape-dependent effects.

\paragraph{MANO Hand Model.}
MANO \cite{MANO2017} is a parametric human hand model that transforms a template mesh using two blend-shape functions based on pose and shape parameters.
First, the shape blend-shape function:
$B_S(\mathbf{\beta}): \mathbb{R}^{|\mathbf{\beta}|}$ 
$ \mapsto \mathbb{R}^{3 \times 778}$ 
maps the shape parameter $\theta$ to a set of per-vertex additive displacements. 
Then, the pose blend-shape function:
$B_P(\mathbf{\theta}): 
\mathbb{R}^s
{\norm{\mathbf{\theta}}} 
\mapsto \mathbb{R}^{3 \times 778}$ models further displacements resulting from the  pose $\theta$.
Adding the displacements to the mean template results in a rest-pose hand mesh $\mathbf{T}_P(\mathbf{\beta}, \mathbf{\theta}) = \bar{\mathbf{T}} + B_S(\mathbf{\beta}) + B_P(\mathbf{\theta})$.

MANO also regresses joint locations in the rest-pose from shape parameters via a linear joint regressor $J(\mathbf{\beta}): \mathbb{R}^{\norm{\mathbf{\beta}}} \mapsto \mathbb{R}^{16}$. 
A set of $4 \times 4$ rigid bone transformations $\{ \mathbf{B}_b \} = \{ \mathbf{B}_1, \cdots, \mathbf{B}_{16} \}$ can be constructed from rest-pose joint locations and relative joint rotations computed from $\mathbf{\theta}$. 

MANO applies standard linear-blend-skinning (LBS) $W(\cdot)$ with the bone transformations $\{ \mathbf{B}_b \}$ and skinning weights $\mathcal{W}$. Transforming $\mathbf{T}_P(\mathbf{\beta}, \mathbf{\theta})$ into the final posed and shaped mesh. Finally, a global translation $\mathbf{t} \in \mathbb{R}^3$ is added to the mesh. 
In summary, MANO models a function $M(\mathbf{\beta}, \mathbf{\theta}, \mathbf{t})$ that takes $\mathbf{\beta}$, $\mathbf{\theta}$ and $\mathbf{t}$ as inputs: 
\begin{align}
\label{eqn:SMPL_func}
    M(\mathbf{\beta}, \mathbf{\theta}, \mathbf{t}) = W(\bar{\mathbf{T}} + B_S(\mathbf{\beta}) + B_P(\mathbf{\theta}); \mathcal{W}, \{ \mathbf{B}_b \}) + \mathbf{t}
\end{align}
The bone transformation $\{ \mathbf{B}_b \}$ are obtained by recursively applying the joint rotations along the kinematic chain.
We denote the $3 \times 3$ rotation matrix representation of joint $b$'s rotation as $\mathbf{R}_b (\mathbf{\theta})$, with $\mathbf{R}_b (\mathbf{0}) = \mathbf{I}, \forall b \in \{1, \cdots, 16 \}$. Let $\mathbf{t}_b \in \mathbb{R}^3$ be the location of rest-pose joint $b$ obtained via $\mathcal{J} (\mathbf{\beta})$. Let $\mathbf{A}(b)$ denote the ordered set of $b$ and its ancestors on the kinematic tree. Let $\bar{b}$ denote the parent of joint $b$. Concretely, the bone transformations $\{ \mathbf{B}_b \}$ from the template mesh to the target pose  are defined as:
\begin{align}
\label{eqn:bone_transformations}
    \mathbf{B}_b &= G_b (\mathbf{\beta}, \mathbf{\theta}) G_b (\mathbf{\beta}, \mathbf{0})^{-1}  \\  
    G_b (\mathbf{\beta}, \mathbf{\theta}) &= \prod_{b^{\prime} \in \mathbf{A}(b)} \begin{bmatrix}   \mathbf{R}_{b^{\prime}} (\mathbf{\theta}) & \mathbf{t}_{b^{\prime}} - \mathbf{t}_{\bar{b^{\prime}}} \\ \mathbf{0} & 1 \end{bmatrix} \\
    \{ \mathbf{t}_b \} &= \mathcal{J}(\mathbf{\beta})
\end{align}
We note that only 16 joints are used for transformation matrix computation, the 5 fingertips are added to the skeleton by a post-processing step.

In this work, we seek to derive the inverse transformation $\{ \mathbf{B}_b^{-1} \}$ (and corollary, $\{ \mathbf{B}_b\}$) using only the keypoints of a posed hand so that the hand surface, parametrized by an implicit surface representation, of the given keypoints can be recovered.
We defer the discussion on how the inverse transformation $\{ \mathbf{B}_b^{-1} \}$ could be computed by our proposed method to Sec. \ref{sec:bio_mech} .

\paragraph{Neural Articulated Shape Approximation (NASA).} 

The goal of NASA \cite{deng2020neural} is to create an implicit representation of the human body which allows articulation so that it can generalize to different poses.
The implicit surface is parameterized by neural networks $\mathcal{O}_w(x|\theta) \to \{0,1\}$, conditioned on the pose descriptor $\theta$.
The network outputs the occupancy probability of a 3D point $x$, where 1 means the point is inside the surface and 0 means the point is outside.
The hand surface can then be obtained via marching cubes \cite{marchingcube} algorithm or used directly for example, for collision detection.
By modeling the surface for each bone separately and positioning them using the inverse bone transformation $\{ \mathbf{B}_b^{-1} \}$, the NASA model learns an implicit representation of pose dependent effects and produces a body model that can be articulated.
Concretely, the learned function is denoted by:
\begin{equation}
    \mathcal{O}_w(x|\theta) = \max_b\{\bar{\mathcal{O}}^b_w(\boldsymbol{B}^{-1}_b x, \mathit{\Pi}^b_w[\{\boldsymbol{B}^{-1} t_0\}])\}.
\end{equation}
where the pose descriptor $\theta$ is defined by a collection of transformation matrices $\{\boldsymbol{B}_b\}_{b=1}^{B}$ that map a posed hand to the canonical pose, and the probability of $\mathcal{O}_w(x|\theta)$ is derived from the maximum occupancy probability across $B$ child occupancy functions $\bar{\mathcal{O}}^b_w(\cdot, \cdot)$ where each represents the body part of a bone $b$. 
For a query point $x$, each child function $\bar{\mathcal{O}}^b_w(\cdot, \cdot)$ maps $x$ to the function's corresponding canonical space by the transformation matrix $\boldsymbol{B}^{-1}_b$ so that the local shape of each body part can be learned. Since each transformation matrix maps a bone from the canonical space to the posed space via a rigid transformation without modeling surface deformation resulted from the pose, the connection at the joint will not be smooth.
To address this, the term $\mathit{\Pi}^b_w[\{\boldsymbol{B}^{-1} t_0\}]$ is used to provide global pose information for each child function by transforming a given reference point $t_0$ to the posed space where $\mathit{\Pi}(\cdot)$ is a learnable projection.
Essentially, by querying the occupancy value $x$ using $\boldsymbol{B}^{-1}_b x$, the NASA model learns a template mesh and the correction based on the global pose with $\mathit{\Pi}^b_w[\cdot]$.
For more details, we kindly refer the reader to \cite{deng2020neural}. 



==> old-abstract.tex <==




    

